iMapper: Interaction-guided Joint Scene and Human Motion Mapping from Monocular Videos

A long-standing challenge in scene analysis is the recovery of scene arrangements under moderate to heavy occlusion, directly from monocular video. While the problem remains a subject of active research, concurrent advances have been made in the context of human pose reconstruction from monocular video, including image-space feature point detection and 3D pose recovery. These methods, however, start to fail under moderate to heavy occlusion as the problem becomes severely under-constrained. We approach the problems differently. We observe that people interact similarly in similar scenes. Hence, we exploit the correlation between scene object arrangement and motions performed in that scene in both directions: first, typical motions performed when interacting with objects inform us about possible object arrangements; and second, object arrangements, in turn, constrain the possible motions. We present iMapper, a data-driven method that focuses on identifying human-object interactions, and jointly reasons about objects and human movement over space-time to recover both a plausible scene arrangement and consistent human interactions. We first introduce the notion of characteristic interactions as regions in space-time when an informative human-object interaction happens. This is followed by a novel occlusion-aware matching procedure that searches and aligns such characteristic snapshots from an interaction database to best explain the input monocular video. Through extensive evaluations, both quantitative and qualitative, we demonstrate that iMapper significantly improves performance over both dedicated state-of-the-art scene analysis and 3D human pose recovery approaches, especially under medium to heavy occlusion.

==> 064_quant_vnect.tex <==
%
%

==> A_leftovers.tex <==
\section{Leftovers - to be deleted at some point}
%
\begin{enumerate}
    \item local 3D poses from \cite{tome2017lifting} (assumes parallel floor upvector) \\
        is sparse in time due to 2D heatmap detection thresholds \\
        yields visibility score $\visibility{\jj}{\timet{i}}$ for each joint $j$ at time $\timet{i}$
        \label{method:init:initialdepth}
    \item filter large jumps in 2D centroids
    \item solve for 3+1 DoF transformation at each video frame (position $\transl$ + rotation around up axis $\rot$), with known intrinsics $\Pi$.
\end{enumerate}
%
%
\mypara{Energy} (initial)
%
\begin{align}
   \underset{\transli{i}, \roti{i}}{\argmin E} = L_{reproj} + w_{smooth} L_{smooth}\ , 
\end{align} $w_{smooth}$ = 0.005 at 10 fps.
      
\mypara{Reprojection term}
\begin{align}
L_{reproj} &= \frac{1}{?} \sum_{\person \in Humans} \sum_{\jj \in Joints^{(\person)}} 
  \big\lVert \visibility{\person,\jj}{\timet{i}} \left(
    \jpostwodt{i} 
      - \Pi 
        \m{M}^{(h)}_{\timet{i}} \jposthreedt{i}
    \right)
  \big\rVert^2\ , 
  \label{eq:e:reproj}
\end{align}
$\m{M}_{\timet{i}} = \mathbf{R}_{\roti{i}} + \transli{i}$, 
~$\mathbf{R}_{\rot} = 
\begin{bmatrix} 
  \cos{\rot} & 0. & -\sin{\rot} \\ 
  0. & 1. & 0. \\
  \sin{\rot} & 0. & \cos{\rot}
\end{bmatrix}$.

%
%
\mypara{Smoothness term} Spatial smoothness ($L_2$ loss on time-difference weighted 3DoF position) \\
%+ additional regularization, if local space ankles don't move, \ie sitting and not walking
\begin{align}
    L_{smooth} &= \frac{1}{?} \sum_{\person \in Humans} \sum_{\timet{i} \in Frames}  \nonumber \\
    &\ \ 
    \frac{1
    %+ w_{ankles}\left(\timet{i}\right)
    }{\timet{i}-\timet{i-1}}
    \big\lVert
      %\transli{i} - \transli{i-1} 
      \m{M}^{(h)}_{\timet{i}} \jposthreedtj{PELV}{i} - \m{M}^{(h)}_{\timet{i-1}} \jposthreedtj{PELV}{i}
    \big\rVert^2 
    \label{eq:e:smooth}
    %w_{ankles} \left( \timet{i} \right) &= \exp^{-2 \max{\left(d_{left\ ankle}\left(\timet{i}\right), d_{right\ ankle}\left(\timet{i}\right)\right)}} \\
    %d_{\jj} \left( \timet{i} \right) &= \big\lVert \jposthreedtj{\jj}{i} - \jposthreedtj{\jj}{i-1} \big\rVert^2
\end{align}




\begin{align}
    &\underset{
      \big\{ \transf{\scenelet}{k} \big\}_{k \in \# scenelets\ chosen}, 
      \big\{ \transf{h}{\timet{i}} \big\}_{h \in Humans, i < \#frames}
    }{\argmin E} = \nonumber \\
    &\ \  L_{reproj} + w_{smooth} L_{smooth} \nonumber \\
    &\ \ \  + w_{intersect} L_{intersect} + w_{occlusion} L_{occlusion}
\end{align}

\mypara{Intersection terms} Two types of intersection implemented using the same point-polygon (quad) distance.
%
\begin{align}
    L_{intersect} &= L_{skeleton-object} + L_{object-object}
\end{align}
%
All skeletons at all times can intersect the objects (oriented bounding boxes) in the scene. We project all objects from top-view to get bounding rectangles. Note, that objects in the same scenelet (\eg couch and table) move together using a single transform $\m{M}^{(scenelet)}$. Pose sequences in the scenelet don't intersect their own objects (not shown in \mbox{Equation~\ref{eq:isec:skelobj}}).
\begin{align}
    & L_{skeleton-object} = \frac{1}{?}
    \sum_{\sceneletk{k}} \sum_{obj_l \in \sceneletk{k}} % for each object in each scenelet
    \sum_{\timet{i} \in Frames} % each frame in the video
    \sum_{\jj \in Joints^{(h)}} % each skeleton joint 
    \nonumber \\
      &~~\max{\left(0, % penalty, if inside
        -\mathcal{D}\left(\m{M}^{(h)}_{\timet{i}}\jposthreedt{i}, % transformed joint position
          ~\transf{\scenelet}{k} \Pi_{top-view} OBB(obj_{l})\right) % transformed object position
      \right)}
    \label{eq:isec:skelobj}
\end{align}
, where $\mathcal{D}$ is the signed 2D point-polygon distance, that's negative on the inside, objects are approximated by their top-view projected bounding rectangle.
%
\begin{align}
    & L_{object-object} = \frac{1}{?}
    % for each pair of scenelets
    \sum_{\underset{k0\neq k1}{\sceneletk{k0},~\sceneletk{k1}}}
    % for each pair of objects not from the same scenelet
    ~~\sum_{\underset{l0 \neq l1}{obj_{l0} \in \sceneletk{k0},~obj_{l1} \in \sceneletk{k1}}} \nonumber\\
    % for each grid point in the top-view rectangle
    &\ \ \sum_{\v{p}_i \in \Pi_{top-view} OBB(obj_{l0})}
         \sum_{\v{p}_j \in \Pi_{top-view} OBB(obj_{l1})} \nonumber\\
    &\ \ \ \max{\left(0, 
           -\mathcal{D}\left(
             \transf{\scenelet}{k0} \v{p}_i, \transf{\scenelet}{k1} \v{p}_j
           \right)
           \right)}
    \label{eq:isec:objobj}
\end{align}

\mypara{Occlusion term} Given a feature point confidence $o^{(h, j)}_{\timet{i}} \in [-1, 1]$, 
\begin{align}
  & L_{occlusion} = 
  \frac{1}{?} % normalize (todo)
  \sum_{\timet{i} \in Frames} % each frame in the video
  \sum_{h, \jj \in Joints^{(h)}} \nonumber\\ % each skeleton joint
  &\ \ 
  \left(- o^{(h, j)}_{\timet{i}}\right) \cdot 
  \min_{\obj{l} \in \sceneletk{k}} % closest [possible] occluder's distance
    \mathcal{O}\left(
      \transf{h}{\timet{i}} \jposthreedtj{j}{i},
      ~\obj{l}
    \right)
\end{align}
...
\begin{align}
    \mathcal{O}&\left(\v{x}, \obj{}\right) = \min_{\m{F} \in \obj{}} \nonumber\\
    &\begin{cases}
        \mathcal{D}\left( \hat{\v{x}}, \m{F} \right) 
        & \text{if } \mathcal{D}\left( \hat{\v{x}}, \v{F} \right) < 0 \textit{;  (-), intersects}
        \\
        \mathcal{D}\left( \hat{\v{x}}, \m{F} \right)
        & \text{if } \exists \hat{\v{x}} \textit{ s.t. } \lVert \hat{\v{x}} \rVert < \lVert \v{x} \rVert \textit{; (+), could be occluded by translation in x} \\
        \min_{\lVert \hat{\v{x}} \rVert < \lVert \v{x} \rVert} \lVert \hat{\v{x}} \rVert - \lVert \v{x} \rVert & \text{can only be occluded by translation in z}
    \end{cases} 
    \\
    &\hat{\v{x}} = \v{x} - \v{n}_{\v{F}} \left(\v{x} - \v{c}_{\v{F}} \right) \v{n}_{\v{F}} % projection to obb face
\end{align}

\subsubsection{Visible interactions}


\if0 % Not used right now
\cma{Possibly obsolete since 2D reprojection fitting...only works for visible interactions}

\mypara{Approach}

\begin{enumerate}
  \item Partition input pose sequence into overlapping scenelets (fixed length in pose centroid arclength). Each scenelet is projected to timeless descriptor space (see \mbox{Subsection~\ref{subsec:interaction_model}}), and resampled (interpolated).
  \item \mypara{Matching} Compute feature distance to all scenelets in the database to create \emph{matches}.
  \item Select \emph{matches} that are characteristic (> $0.3$) and close in feature space (< $0.1$).
  \item Align matches to video poses using a weighted falloff of positions and forwards. Position and forward of skeleton pose in the middle sample of the scenelet is more important, than the sample at the ends. Each scenelet is 15 samples large. Note, this has nothing to do with the occurrence time of the scenelet in the recording.
  \item \mypara{Evidence volume} Sum up the aligned local environment statistics (histograms) in a discretized evidence volume. The volume is 4D, categories, top view position ($\jposthreed_{x, z}$), orientation ($\rot$).
  \item \mypara{Candidate generation} Extract characteristic patches, compare evidence maps of these patches in pose-local space, candidates are the nearest neighbours based on distance
  \begin{align}
     &\mathcal{D}\left(query\ patch, candidate\ patch\right) = \sum_{category,~x,~z} \\
     &\big\lvert 
        \textsc{Normalize}\left(\mathbf{V}_{query\ patch}\right)
       - \textsc{Normalize}\left(\mathbf{V}_{candidate\ patch}\right)
     \big\rvert
  \end{align}
  
  \begin{align}
      \textsc{Normalize}\left(\m{V}\right) &= \frac{
        \textsc{Collapse}\left(\mathbf{V}\left(category, x, z, \rot \right)\right)
      }{
        \underset{x, z}{\max}~\textsc{Collapse}\left(\mathbf{V}\left(category, x, z, \rot \right)\right)
      }
      \\
      \textsc{Collapse}\left(\mathbf{V}\right) &= \underset{\rot}{\max}\m{V}\left(category, x, z, \rot \right)
  \end{align}
  %\item \mypara{Selection}
  %\item \mypara{Refinement of placement} MCMC?
  %\item \mypara{Refinement of skeleton path} (rerun from (1))
\end{enumerate}
\cma{Possibly: use these candidates in \mbox{\ref{sec:method:occluded}.\ref{method:method:refine}}}.
\fi

\subsubsection{Occluded interactions}\label{sec:method:occluded}

\begin{enumerate}
    \item \textbf{occluded motion} Select all "long" gaps in time, where we didn't get any local 3D poses from \cite{tome2017lifting}, because of a conservative 2D feature point detection threshold ($10^{-4}$ on \cite{wei2016}'s feature maps). We are very conservative, otherwise we get poses "lying on bed" 2m above ground where ankles/knees not visible. In practice: a gap is longer than a second, which is 10 frames at 10 fps. Todo: fit [walking] scenelets to walking parts that have more than 50\% missing poses (starting where in time?).
    \item \textbf{iterative fill} Using the initial depth estimates from above, iterate over all gaps in time in depth order (average depth of first and last visible pose).
    \item \textbf{scenelet fitting} Search through the pigraphs database of scenelets (ideally the characteristic ones, right now not, which is a problematic point from the method's point of view.) Fit each of them to the unoccluded joints.
    Unknowns: x-z position and orientation around y, for each rigid scenelet (objects + poses).
    Energy: 2D reprojection of visible joints (Equation~\ref{eq:e:reproj}), 3D spatial smoothness when connecting to static path from \mbox{\ref{sec:method:init}.\ref{method:init:initialdepth}} (Equation~\ref{eq:e:smooth}) + occlusion consistency of joints (can the objects in this scenelet occlude the joints that were not visible in the video). Implemented in parallel on the GPU, used to run at 1 scene/second, where we have 50 scenes. Todo: implement occlusion term. \label{method:method:search}
    \item \textbf{z-refinement} Given a scenelet that fills a gap in time, re-optimize the initially placed local 3D poses in \mbox{\ref{sec:method:init}.\ref{method:init:initialdepth}} and the already placed scenelets (from step \ref{method:method:search}), so that the poses don't intersect the objects of the scenelets, and the objects don't intersect each other (if different category, or orientation; tables can intersect, couches can intersect if they are facing the same way).
    Unknowns: z of each scenelet, z of each local 3D pose.
    Energy: 2D reprojection; skeleton-object intersection (2D top-view point-polygon distance); object-object intersection (2D top-view point-polygon distance, where each polygon is rasterized to a meshgrid of points at 10cm); visibility consistency; object-object relative arrangement term (todo). \label{method:method:refine}
    \item \textbf{iterate} Go to \ref{method:method:search} for next gap.
    \item \textbf{Stop}, if no more gaps. Optional: re-iterate to recover from initial mistakes (occlusion consistency biases towards large objects closer to the camera)
    \item Optional: Fit scenelets to visible poses that were placed in \mbox{\ref{sec:method:init}.\ref{method:method:initialdepth}} so that we can render the visible interactions more plausibly (sit on couch, and not behind it).
\end{enumerate}

\depr{
\begin{enumerate}
    \item calibrate camera: make sure ground plane is marked + we can project 3D points to the camera view
    \item perform proposal generation (using RCNN?) and insert fuzzy voxel candidates based on that. Place the voxels on the ground. Have to keep an aggressive threshold for this stage.
    \item perform image space marker heat map generation (using DeepCut?) and fit to animation clips/blended frames. Use the voxels to give indications of possible occlusion
    \item Use the motion path estimated in \# 3 to cleanup voxel estimated in \# 2. If 'sit' is detected, then likely to have chair/sofa there; if walking, then the volume around is likely to be free; is not a straight path, then some object around the corner, etc.
    \item Iterate 3-4
\end{enumerate}
}

\paul{old:}

These scenelets should be consistent with both the video and each other, which we express with an energy that penalizes inconsistency:
\begin{equation}
\argmin_{P, \mathcal{X}} L = w_r L_r + w_o L_o + w_s L_s + w_c L_c,
\end{equation}
where $L_r$ is the reprojection error, $L_o$ penalizes occlusions of skeleton joints in the video that are not explained by the scenelets, $L_s$ encourages a smooth human performance, without discontinuities, and $L_c$ penalizes intersections between objects in different scenelets. Our goal can then be re-stated as minimizing this energy over possible choices of scenelets and their poses $P = [p_1^T, \dots, p^T_{n_v}]$.
%, where $m_v = {\mathbf{1}^T \mathcal{X} \mathbf{1}}$ is the number of chosen scenelets.

\mypara{Reprojection error}
\begin{equation}
L_r = \sum_{(l,t)} \sum_{i} \sum_{k} \mathcal{X}_{lt} \left\|\Pi T(p_t) s^{li}_k - u^{t+i}_k \right\|_2^2 v^{li}_k(p_t)\ c^{t+i}_k,
\end{equation}
where $T(p_t)$ is the transformation matrix from the local coordinate frame of a scenelet at $p_t$ to world space, and $v^{li}_k(p_t)$ is the visibility of joint $k$ in frame $i$ of scenelet $l$ given the scenelet pose $p_t$. This visibility includes possible occlusions from other scenelets.

\mypara{Occlusion error}
\begin{equation}
L_o = \sum_{(l,t)} \sum_{i} \sum_{k} \mathcal{X}_{lt} H(v^{li}_k(p_t), c^{t+i}_k),
\end{equation}
where $H$ denotes the cross entropy.

\paul{or:}

\begin{equation}
L_o = \sum_{(l,t)} \sum_{i} \sum_{k} \mathcal{X}_{lt} \left\|v^{li}_k(p_t) - c^{t+i}_k\right\|_2.
\end{equation}

\mypara{Smoothness term}
\begin{equation}
L_s = \sum_{(l,t)} \sum_{i} \sum_{k} \mathcal{X}_{lt} \left\|v^{li}_k(p_t) - c^{t+i}_k\right\|_2.
\end{equation}


\subsection{from overview}
%object configurations with humans interacting with them (see \cite{pigraph}). \duygu{this is where I stop} 
%Incrementally build the scene. 

\mypara{Method shorter}\\
(a) pre-process: determine characteristic scenelets in the dataset \\

(b0) init path: Denis' sparse local poses to approximate global poses 
\cma{(terms: (reproj, spatial smooth))} \\

(b1) scenelet fit: fit scenelets to each time interval (both partially hidden and visible), 
\cma{(terms: (reproj, spatial smooth, local occlusion))} then \\

(b2) scenelet selection: select a subset of these scenelets that are i) characteristic ii) match the 2d fps well iii) do not overlap in time (or overlap only minimally) - this subset does not explain the entire scene yet - especially more occluded parts may not be explained yet \cma{(terms: (reproj, spatial smooth?, local occlusion; charness, overlap penalty))} \\

(c) optimize depth of placed scenelets
\cma{(terms: (reproj, spatial smooth, global occlusion, skel-object intersection, object-object intersection))} \\

(d) iterate (b1\dots c) keeping the previously placed scenelets fixed and using them for occlusions\\

\mypara{Method outline}
\begin{enumerate}
    \item \textbf{pose detection} 2D features from \cite{wei2016}, local 3D poses from \cite{tome2017lifting}. \label{intro:method:one}
    \item \textbf{visible motion} Initial guess of path depth and pose height from input local 3d poses using re-projection term and spatial smoothness with temporal decay. Works, if we occasionally see an unoccluded pose between occlusions. For long "gaps" it will start sliding in depth to confuse our initial ordering, which we don't know, if is a problem yet. \label{intro:method:initialdepth}
    \item \textbf{occluded motion} Select all "long" gaps in time, where we didn't get any local 3D poses from \cite{tome2017lifting}, because of a conservative 2D feature point detection threshold ($10^{-4}$ on \cite{wei2016}'s feature maps). We are very conservative, otherwise we get poses "lying on bed" 2m above ground where ankles/knees not visible. In practice: a gap is longer than a second, which is 10 frames at 10 fps. Todo: fit [walking] scenelets to walking parts that have more than 50\% missing poses (starting where in time?).
    \item \textbf{iterative fill} Using the initial depth estimates from above, iterate over all gaps in time in depth order (average depth of first and last visible pose).
    \item \textbf{scenelet fitting} Search through the pigraphs database of scenelets (ideally the characteristic ones, right now not, which is a problematic point from the method's point of view.) Fit each of them to the unoccluded joints.\\
    Unknowns: x-z position and orientation around y, for each rigid scenelet (objects + poses).\\
    Energy: 2D reprojection of visible joints, 3D consistency when connecting to static path from \ref{intro:method:initialdepth} + occlusion consistency of joints (can the objects in this scenelet occlude the joints that were not visible in the video). Implemented in parallel on the GPU, used to run at 1 scene/second, where we have 50 scenes. Todo: implement occlusion term. \label{intro:method:search}
    \item \textbf{z-refinement} Given a scenelet that fills a gap in time, re-optimize the initially placed local 3D poses in \ref{intro:method:initialdepth} and the already placed scenelets (from step \ref{intro:method:search}), so that the poses don't intersect the objects of the scenelets, and the objects don't intersect each other (if different category, or orientation; tables can intersect, couches can intersect if they are facing the same way).\\
    Unknowns: z of each scenelet, z of each local 3D pose.\\
    Energy: 2D reprojection; skeleton-object intersection (2D top-view point-polygon distance); object-object intersection (2D top-view point-polygon distance, where each polygon is rasterized to a meshgrid of points at 10cm); visibility consistency; object-object relative arrangement term (todo).
    \item \textbf{iterate} Go to \ref{intro:method:search} for next gap.
    \item \textbf{Stop}, if no more gaps. Optional: re-iterate to recover from initial mistakes (occlusion consistency biases towards large objects closer to the camera)
    \item Optional: Fit scenelets to visible poses that were placed in \ref{intro:method:initialdepth} so that we can render the visible interactions more plausibly (sit on couch, and not behind it).
\end{enumerate}

\mypara{Contributions} Core to our algo is 
% a novel interaction consistency energy that ensures space-time ... 
%and consistent camera space projection .. characteristic poses (***let us work on the list .. ***)

\begin{enumerate}
    \item Occluded 3D, world-space pose estimation (plausible and scene-consistent motion, not super-tight reconstruction) - consistent camera space projection (of human joints (works) and objects (todo)).
    \item Iterative refinement of depth estimates (monocular)
    \item Interaction detection (occluded (works) and not occluded (hopefully works)) via characteristic pose sequences. \textit{Not all parts of a performance contain interactions. Determining, when interactions happen is difficult with missing data.}
    \item Varying time scales (quick sit vs. long sit) - via projection to descriptor space \cma{only used for unoccluded interactions right now}
    \item Consistent scene synthesis - separate interactions need to be combined into a consistent scene and performance. i) number of objects ii) object categories iii) objects' placement and orientation iv) realisitc room layouts (arrangement term) v) compatible performance (sit on couch and not next to it)
\end{enumerate}





\cma{I'm not sure, if we use the evidence volume in the end}

\paul{from introduction:}
\duygu{I merged parts of the following to the introduction}
%para4
%Augmenting algorithms with a similar human perception Transferring the above to an algorithm requires overcoming several challenges: 
%1) Both Interactions and objects are often are partially occluded.
%2) Not all parts of a performance contain interactions. Determining, when interactions happen, is difficult with missing data.
%3) Separate interactions need to be combined into a consistent scene and performance  
%4) Depth estimate is approximate at best. But ordering information is more reliable. (e.g.person walks in front of a sofa)
%5) different speed of interaction and variability
%
Our goal is to develop a computational algorithm that masters a similar perception as described above. Given an input video with partially tracked human 2D joint locations over time, the desired output consists of a plausible scene configuration and a captured human performance that is compatible both with the inferred scene and the input data. 
%
To achieve this, we need to overcome several challenges. First, both interactions and objects in the scene are often partially occluded in the input video. Second, humans interact with the same object configurations at different speeds and with some variations, making it difficult to match them to a pre-defined set of interactions. Third, some human actions are less characteristic than others. For example, walking along a path is only loosely affected by the objects around it. Determining when an useful interaction happens is another hurdle. Finally, when separate interactions are detected they need to be combined into a consistent scene and human performance. We observe that monocular depth estimates are at best approximate whereas ordering information is more reliable (\eg person walking in front of a sofa). %Such information needs to be utilized to produce the final output.

\paul{end from introduction}


\if0
\begin{itemize}
\item detecting interactions (object-pose) -- animation sequence matching in space-time
\item b) creating evidence volume: this is the step we go from (detected) interaction -> occupancy/per-category grid data
\item c) evidence volume -> object map: this is the step we get from fuzzy occupancy map to crisp object map
\item d) take crisp occupancy map + scene statistics to create final scene
\end{itemize}
\fi

Our method takes a track of human joint locations over time as input. In our experiments, these are extracted from a monocular video shot by a static camera with known intrinsics, but other sources, such as motion trackers, may be used as well. Using a database of short pose sequences and pose-object relationships (which we call \emph{scenelets}), our method generates a global 3D scene which is compatible with the input track. We introduce the main parts of our method below, and detail them in the following sections. 

% Our method takes a monocular video that has been captured through a video camera whose position with respect to the world is static at capture time and whose intrinsic properties are known. Using a database of atomic 3D local poses and pose-object relationships (which we call \emph{scenelets}), our method generates a global 3D scene and 3D skeletal motion which is compatible with the input video. We introduce the main parts of our method below, and detail them in the following sections. 

%\mypara{Preprocessing} % as niloy said, calling it preprocessing makes it seem like the contributions in here are less relevant
\mypara{Scenelet extraction}
We create a scenelet database from the raw data captured by Savva et al.~\shortcite{savva2016pigraphs}. Scenelets capture short interaction sequences of a human with neighboring objects. They consist of a short sequence of joint locations, referred to as {\em pose sequence}, and a set of objects within interaction distance. The scenelet database models a large range of possible relationships between object arrangements and human skeleton motions. To filter out accidental or unreliable relationships, we determine how characteristic each pose sequence is for the objects in the scenelet and their relative locations. We start by defining a pose descriptor (see also \cite{geomfeatures:2017:wacv}) that is more descriptive than raw joint locations and invariant to location and orientation of the skeleton. Next, we remove the time dependence from the pose sequences in the raw dataset. Specifically, motions such as sitting and walking can be performed at various speeds without changing the interacting objects, so we would like our scenelets to be invariant to time. We chop up the arbitrary length pose sequences in the raw dataset to sequences of fixed arc length in the space of skeleton locations (taken to be the pelvis location) and re-sample this sub-sequence with a constant sampling rate in the space of pose descriptors and skeleton locations, which we call the \emph{descriptor-location} space,. This factors out time, while ensuring that we do not miss any important motion sequences. Finally, we  estimate object occurrence density in the space of pose descriptors and define pose sequences that have a consistent local object arrangements as characteristic poses.

%We create a scenelet (local space-time contexts of pose-geometry interaction with fixed temporal length) database from the raw data captured by Savva et al.~\cite{savva2016pigraphs} \cma{it's not space-time anymore, we need a name for the augmented human motion space composed of the combined space of skeleton position, skeleton forward and skeleton descriptors. The descriptors are following the findings in \cite{geomfeatures:2017:wacv}, not angles but joint distances}. Specifically, our goal in this step is to determine characteristic pose sequences, local object arrangements and their relationships. We start by chopping an arbitrary length motion capture into fixed length short sequences. We then create clusters out of such short-length motion sequences through a similarity match~\cite{Wang_2016_CVPR}. We analyze the object occurrence statistics for each cluster, and define poses that have a consistent local object arrangements as characteristic poses. Finally, we build a kd-tree of scenelet pose descriptors to help optimal search at runtime \cma{kd-tree can't take weighted distance, so we do exhaustive L2 distance in pose descriptor space with Gaussian falloff centered around the half arclength of the scenelet}.

%As part of the data preprocessing, we also generate object-to-object relative location and orientation statistics given 3D indoor scenes~\cite{fisher2015actsynth} to be later used during scene synthesis. 


\mypara{3D motion reconstruction} Starting from input monocular video, we estimate per-frame 2D joint location heat maps and corresponding single 3D poses~\cite{tome2017lifting}. These poses, however, come in local coorodinate spaces with the pelvis joint being at the origin.  We filter out ambiguous 2D pose detections if the correspoding joint  placements strongly disagree with previous and later frames.  
%
\if0
~\ersin{is this correct?} \cma{they already do that heatmap filtering for us. We filter out erroneous but consistent 2D skeleton detections (where they placed a large fraction of the 2D joint positions to depict a 2D skeleton, but it's not consistent with the previous and the next frame. They don't have time consistency, each frame is solved separately. We throw away frames, where the average 2D centroid of the non-filtered out heatmap detections (which usually form a skeleton) is too far away from the previous frame's 2D skeleton centroid. Occasionally their 2D skeleton jumps 200 pixels, we detect that by Winsorziation \url{https://docs.scipy.org/doc/scipy-0.13.0/reference/generated/scipy.stats.mstats.winsorize.html}, but don't clamp it to a plausible value, just throw away the frame}). 
\fi
%
We then jointly solve all individual static poses from the remaining frames such that consecutive 3D translations between frames are smooth (i.e., $l2$ loss), by optimizing over 3D translations of the static poses in space and their rotation around the up-axis. The resulting globally smooth and continuous motion sequence is our initial 3D motion reconstruction.

\mypara{Pose sequence-guided scene synthesis}
We use the initial
%continuous \cma{it's not continuous due to the filtering above}
3D motion reconstruction to seed a search into our scenelet database. We use a sliding window in the space of pose locations, re-sampled in the descriptor-location space,
%\cma{in the augmented space}
to clip constant length short pose sequences and match them with characteristic pose sequences in our database. We then transfer the consistent object arrangements corresponding to these sequences to the local coordinate frame of the sliding window.
%
Note that multiple scenelets with different object arrangements may match the same sliding window and neighboring matches are not guaranteed to be consistent, they may contain intersecting object for example. We solve this problem by accumulating the evidence for an object of a given type being placed at a given location in a volume. In addition to this evidence volume, plausibility of the created scene is measured using a probabilistic model of object occurrence and arrangement~\cite{fisher2015actsynth}, that is used together with the evidence volume to place objects.

%We can then place objects by sampling this volume, for example placing objects at maxima of the volume.
%When such characteristic poses have consistent object distributions around them, we transfer these distributions to the scene around the locale of the motion sequence that is matched to the characteristic pose.
%Note that, there might be many poses within a locale that point to the same characteristic pose, and thus to the same type of object distributions multiple times since actions span a finite time (\textit{e.g.}, sitting on a chair is not an instantaneous action, rather it spans a considerable length of time). We solve such cases at object placement time: when we retrieve and place an object into the scene based on that object type's maxima, we use the watershed transform to remove that mode of the distribution from the global distribution of the type before retrieving and placing the next instance. We weight this two step \emph{(1)~retrieve and place object - (2)~update category distribution} process with the scene-object relationship Bayesian network probabilities learned during the preprocessing step from realistic scenes.

% lets leave this out for now
%\mypara{Joint motion-scene refinement} \ersin{This is pending (AFAIK, it is pending implementation as well based on the bullet points below?). I will wait until someone confirms my writing above and then proceed to write this final element in overview as well. By then we might have more solid implementation details about this. } \cma{The above is great, quite spot on except the lack of time dimension which we recently invented and the heatmap, per-joint 2D filtering, which they do already. \\
%And yes, we don't know, if we'll get to re-optimizing the motion. Maybe we can do it in top-view 2D with signed distance to rectangles, which would prevent chairs being under tables, but would avoid the difficulties of constructing 3D signed distance fields from sets of unoriented mesh faces.}.



\begin{comment}

========================================

\ersin{Raw bullet points. We can nuke them once done with overview. }

Input: \\
a) Monocular video (w/ fixed camera with known intrinsics) \\
b) 3D local poses


Output: \\
a) Synthesized 3D scenes with placed and oriented models that are plausible w.r.t. the observed skeleton motion \\
b) Different types of output scenes for the same input motion(office, living room)
c) Corrected global skeleton path (pending) \\


Method: \\
\mypara{Database creation}
\begin{enumerate}
    \item Create scenelets (local space-time contexts of pose-geometry interaction)
    \item (pending) Project to space without time
    
    \item Identify characteristic pose sequences, local object arrangements and their relative relations (occupancy histograms)
    \item Robustify pose matching descriptor (weigh angles?)
    \item cite~\cite{Wang_2016_CVPR}
    
    \item Create augmented global scene (object*) statistics (\cite{fisher2015actsynth})
    \item Create object-object relative position (and orientation?) statistics (GMMs) (\cite{fisher2015actsynth})
\end{enumerate}

\mypara{Global 3D pose}
\begin{enumerate}
    \item Input 3D local pose sequences
    \item Filter erroneous 2D detections
    \item Find 3D translation and 1D (around up-axis) rotation of input local poses
    \item Consecutive 3D translations should be close (L2 smoothness)
    \item (Scipy optimizer (L-BFGS approximated Hessian), Tensorflow)
\end{enumerate}

\mypara{Pose matching}
\begin{enumerate}
    \item Pre-processing: build KDTree of [weighted] scenelet pose descriptors
    \item For each frame, build pose descriptor from input path with sliding window (K=15) in time (or space (pending))
    \item Fetch closest characteristic poses in database
\end{enumerate}

\mypara{Scene synthesis}
\begin{enumerate}
    \item Splat Gaussians for each matched scenelet into the 4D probability volume with dimensions: \\
      \#categories $\times$ 10cm resolution 2D grid $\times 45^{\circ}$ resolution orientation grid
    \item normalize volume
    \item Weigh per category slices by Bayes Network probability of having one or more objects of that category \label{enum:scenesynth}
    \item \emph{Add} GMMs for all object instance pairs (both ways), set minimum to 0.1, \emph{multiply} with volume
    \item Pick highest volume maximum (or weighted sample for variety)
    \item Place object without intersection (pending: optimize jointly)
    \item Identify corresponding probability mountain with watershed, remove from volume
    \item Repeat from \mbox{Step~\ref{enum:scenesynth}} until Bayes Network score decreases or the placed object volume score is below threshold (pending)
    \item Optimize final placements (pending)
    \item Add objects not related to motion (Todo)
\end{enumerate}

\mypara{Path refinement (pending)}
\begin{enumerate}
    \item Fix pose heights, optimize for 2D top-view skeleton location
    \item Fix placed objects
    \item For each y-slice of space above ground, add smooth cost for joint-rectangle intersection 
    \item Alternative: 3D distance field
    \item Risk: bad/noisy local 3D pose is impossible to fit into space
\end{enumerate}
========================================

\end{comment}


\subsection{More from overview}
\paul{old}:

%
%to single frames or short sequences of the input video.
In each frame of the video, we detect the 2d skeleton of the actor, consisting of $n_j$ joint locations, using the method by Tome et al.~\cite{tome2017lifting}. Which of the two models we fit to a given part of the video depends on two factors: the amount of joint occlusion observed in the video (i.e. the strength of the joint signal) and the presence of object interactions.

For parts of the video that contain an unoccluded human performance without object interactions, we can fit static skeletons to each frame. Since the degrees of freedom for human poses is smaller than for human-object interactions, the space of possible human poses can be covered more accurately than the space of possible human-object interactions. Thus, fitting static skeletons to the video gives us better performance in unoccluded sequences that do not contain interactions.

Video sequences that contain interactions with objects are better modeled with scenelets. Scenelets both allow us to populate the scene with objects involved in interactions and explain occlusions of joints due to these objects. Joint occlusions can thus help us in the choice and placement of scenelets: for a given video sequence we would like to choose and place a scenelet such that the scenelet objects explain the joint occlusions observed in the video sequence.

%


For parts of the video that contain an unoccluded human performance without object interactions, we can use more traditional skeleton pose fitting to obtain synthesized joint positions. Since the degrees of freedom for human poses is smaller than for human-object interactions, the space of possible human poses can be covered more accurately than the space of possible human-object interactions. Thus, fitting 3d skeletons to the video gives us better performance in unoccluded sequences that do not contain interactions.

Video sequences that contain interactions with objects are better modeled with scenelets. Scenelets both allow us to populate the scene with objects involved in interactions and explain occlusions of joints due to these objects. Joint occlusions can thus help us in the choice and placement of scenelets: for a given video sequence we would like to choose and place a scenelet such that the scenelet objects explain the joint occlusions observed in the video sequence.

We fit these two types of models to the joint locations observed in the video using an energy function that also ensures the models fitted to different parts of the video are consistent with each other. This fitting energy is described in Section~\ref{sec:fitting_energy}.

\paul{older}:

%para 5: our solution
Technically, we solve the above challenges in three steps: first, we analyze the input scene-action dataset to identify {\em discriminative \sout{actions} \cma{motion sequences?}} that can be reliably linked to 
{\em characteristic scenelets}; second, we propose a novel space-action parametrization that allows us to retrieve scenelets based on human actions while being largely robust to the speed and marginal variation of the corresponding action; and finally, a scene synthesis algorithm that  selects and arranges the retrieved candidate scenelets to plausibly explain the input human actions. 
%
Note that our approach does not expect an explicit labeling of actions, but rather rather determines characteristic ones based on action-object correlations in the input database. 


Figure~\ref{fig:teaser} shows a plausible scene layout proposed by our algorithm that explains the input joint locations over time. \ersin{We will discuss quantitative evaluation/results summary here. I will write it once we have those in place.}


\ersin{Aron's Comments about contributions of scenelet generation:\\
- representing the motion of the human in the human-scene interaction database \emph{without} the time dimension, in the augmented space composed of $\langle$ \text{pose location}, \text{pose descriptor (angle related triangle distances)}, \text{pose forward} $\rangle$. We take overlapping, smoothed, resampled, equal length (arclength) series of points (lines) in this space in order to be invariant to how long parts of interactions take in time. \\
E.g. standing up slowly versus quickly will be represented the same way, if the integral of the angular displacements, pose forwards, and pelvis position changes are the same. 
Wiggling around in the chair seat compared to sitting still keeps a bit of the interesting details due to the changes in the pose descriptor sub-space, since the pose descriptor changes during leaning back and forth on the chair. \\
- clustering poses based on their local object layout context in the database (top-view radial histograms) allows us to identify poses, that are close to each other in the above mentioned, augmented space with time projected away, and have similar nearby objects relative to the pose location and forward. This allows us to identify characteristic poses and their typical local layout histograms. \\
The recognition of the characteristic poses allows us to splat only important scenelets into the probability volume that will then be optimized for scene synthesis, and allows us to reduce the noise by spurious pose matches mostly coming from walking and standing which have ambiguous local contexts. 
The characteristic local layouts (typical histograms) should allow us to weigh the importance of the scenelet objects we splat into the volume based on how typical they are to the poses in the matched part of the human motion reconstruction.}


\begin{comment}
Scene reconstruction from sparse information can be seen as an instance of constrained scene synthesis: missing scene information is synthesized given the existing information as constraints.
%
In our settings, we use a captured pose sequence as constraints for a scene synthesis based on information from existing scene datasets.
%
\duygu{do we really need the following sentence here? maybe it can go into the next paragraph}
We do not re-project the synthesized scene to the video to verify the placed objects, since the video only shows a small subset of scene objects.




We can roughly distinguish two types of constraints on our scenes that we can extract from these interactions. First, characteristic interactions with objects, like sitting on a sofa, tell us about the location, orientation and type of objects being interacted with. Second, more general actions, like walking around an obstacle, tell us about occupied and empty spaces in the scene.
%Two concepts: (i) actions tell us about location and type of objects being interacted with; (b) walking paths (goes around) tell us occupied vs empty spaces; 




Just observing pose over time tells us something about the scene. Such pose sequence to scene synthesis hasn't been investigated.
With enough data, object to object correlation has been investigated. However pose to object has been little investigated expect for pi graph.
Time carries lots of information. How we approach a stool versus arm chair is different. Just looking at a single pose we can't differentiate this.
Technically we solve this by proposing canonical poses with associated objects.
And using arc length parametrrizatiom.



% this should be before giving the method overview, this is part of the motivation that reconstructing poses is easier than  reconstructing the scene (necessary to complete the argument started in para2)
Monocular pose estimation is a well studied problem that is less ill-defined than monocular scene acquisition, since the space of human body poses can be modeled with less ambiguity and less degrees of freedom than the space of possible scenes.
%The space of human bodies and poses is much more well studied and modeled.
% The space of possible human poses also has less ambiguity and less deg. of freedom than the space of possible scenes when being reconstructed.
%
This allows recovering body poses even under moderate occlusion and the temporal continuity of poses can be used to further stabilize extracted pose sequences.
%The recoverved poses can then be used to regularize scene estimation. 
% Talk about time and space. 
%Under moderate occlusion, it is still possible to get human body keypoints and also body poses. 


%para 3: describe the formulation as an instance of scene synthesis: actions provide some information; rest coming from scene statistics + object colocation; emphasise we do not really project back to video as there is no video information due to occlusion
\duygu{shall we reverse the order of sentences here, linking to the above paragraph, we can say we want to utilize the less ambiguous space of human poses to help resolve the scene ambiguity. This becomes a constrained scene synthesis problem where the constraints come from human poses}
Scene reconstruction from sparse information can be seen as an instance of constrained scene synthesis: missing scene information is synthesized given the existing information as constraints.
%
In our settings, we use a captured pose sequence as constraints for a scene synthesis based on information from existing scene datasets.
%
\duygu{do we really need the following sentence here? maybe it can go into the next paragraph}
We do not re-project the synthesized scene to the video to verify the placed objects, since the video only shows a small subset of scene objects.

%para 4: describe the main idea: motion snippets; action types; action > 'scenelets'
\paul{This paragraph (method overview) should probably be completed once we know the terms, etc. used in the method}

Geometry helps estimate occlusion of body parts (joints), which robustifies pose estimation.
\paul{will we improve pose estimation?}


%para5: evaluation
We extensively evaluated .. + comparison


\cma{
Input: Monocular video + local 3D pose sequence (\cite{tome2017lifting}) \\
Preproc: global 3D pose (reprojection, outlier detection, spatio-temporal smoothness) \\
Goal: From global 3D pose ("path") to plausible scene arrangements \\
Ill-posed: some pose sequences are more informative than others \\
Scene synthesis seeded by characteristic pose sequences and characteristic local object arrangemenets \\
}

Main contributions:
\begin{itemize}
    \item Identification of characteristic pose sequences and local object arrangements
    \item Pose matching based on space curves (pending, reference?)
    \item Use these as seed for human motion guided scene synthesis 
    \item Global scene coherence via 
    \begin{enumerate}
        \item 3D probability volume (x, z, theta)
        \item (Augmented Discrete Bayesian Network (from \cite{fisher2015actsynth})
        \item (GMM-s from \cite{fisher2015actsynth})
    \end{enumerate}
    \item \depr{voxelization robustifies pose estimation (and global pose \ie tracking)} \duygu{similar to Paul's comment above, this contribution can be claimed if we only improve pose estimation?}
    \item \depr{global pose estimation + action reasoning improves geometry estimation}
\end{itemize}

\end{comment}

\subsection{From Scenelets and Skeletons}

\mypara{Time invariance}

- location space: scenelets represent fixed neighborhoods in location space, since objects are localized in space

- descriptor-location space: we want to capture the skeleton path, as well as the poses along the path. location captures path, descriptor poses along path

We start with the PiGraphs dataset~\cite{savva2016pigraphs} as a source of information about human-room interactions. This dataset provides raw skeleton joint trajectories in reconstructed 3D rooms with labeled objects. \paul{todo: a little bit more info about dataset (statistics like average sequence times, capture device etc.)} From this dataset, we want to extract a set of short interaction sequences that are characteristic for an object, or an arrangement of objects, and that can be summarized by fixed-length descriptors. We call these short interaction sequences \emph{scenelets}.

\subsection{From Scene Synthesis}

\paul{how are unoccluded sequences defined? enough joints visible?}
\cma{Denis discards some based on an average visibility threshold, and I discard some that jump too much in screen space or in local 3D space or are invalid poses (feet above head)).}

Initially, we do not know if any given video sequence contains interactions. Therefore, we start by fitting 3d skeletons to all unoccluded sequences of the video. Then, we fit scenelets to the video, as described above.
%
\paul{to which parts?}
%
As discussed in Section~\ref{sec:interaction_prior}, high charness in a scenelet indicates the presence of an object interaction. We therefore keep scenelets with high charness and discard scenelets with low charness in favor of the fitted 3d skeleton.

\paul{todo: for scenelets we fix the height z to the height of the skeleton placed at the same frame and optimize only over $(x,y,\theta)$}

\begin{enumerate}
    \item \textbf{occluded motion} Select all "long" gaps in time, where we didn't get any local 3D poses from \cite{tome2017lifting}, because of a conservative 2D feature point detection threshold ($10^{-4}$ on \cite{wei2016}'s feature maps). We are very conservative, otherwise we get poses "lying on bed" 2m above ground where ankles/knees not visible. In practice: a gap is longer than a second, which is 10 frames at 10 fps. Todo: fit [walking] scenelets to walking parts that have more than 50\% missing poses (starting where in time?).
    \item \textbf{iterative fill} Using the initial depth estimates from above, iterate over all gaps in time in depth order (average depth of first and last visible pose).
    \item \textbf{scenelet fitting} Search through the pigraphs database of scenelets (ideally the characteristic ones, right now not, which is a problematic point from the method's point of view.) Fit each of them to the unoccluded joints.
    Unknowns: x-z position and orientation around y, for each rigid scenelet (objects + poses).
    Energy: 2D reprojection of visible joints (Equation~\ref{eq:e:reproj}), 3D spatial smoothness when connecting to static path from \mbox{\ref{sec:method:init}.\ref{method:init:initialdepth}} (Equation~\ref{eq:e:smooth}) + occlusion consistency of joints (can the objects in this scenelet occlude the joints that were not visible in the video). Implemented in parallel on the GPU, used to run at 1 scene/second, where we have 50 scenes. Todo: implement occlusion term. \label{method:method:search}
    \item \textbf{z-refinement} Given a scenelet that fills a gap in time, re-optimize the initially placed local 3D poses in \mbox{\ref{sec:method:init}.\ref{method:init:initialdepth}} and the already placed scenelets (from step \ref{method:method:search}), so that the poses don't intersect the objects of the scenelets, and the objects don't intersect each other (if different category, or orientation; tables can intersect, couches can intersect if they are facing the same way).
    Unknowns: z of each scenelet, z of each local 3D pose.
    Energy: 2D reprojection; skeleton-object intersection (2D top-view point-polygon distance); object-object intersection (2D top-view point-polygon distance, where each polygon is rasterized to a meshgrid of points at 10cm); visibility consistency; object-object relative arrangement term (todo). \label{method:method:refine}
    \item \textbf{iterate} Go to \ref{method:method:search} for next gap.
    \item \textbf{Stop}, if no more gaps. Optional: re-iterate to recover from initial mistakes (occlusion consistency biases towards large objects closer to the camera)
    \item Optional: Fit scenelets to visible poses that were placed in \mbox{\ref{sec:method:init}.\ref{method:method:initialdepth}} so that we can render the visible interactions more plausibly (sit on couch, and not behind it).
\end{enumerate}

- scenelet characteristicness: max of object characteristicness over all bins

- normalization for similar pose, similar location (based on density of poses in descriptor-location space, for each scene separately)

- normalization for min. amount of evidence (linear falloff of scenelet characteristicness below min. evidence = pose density in descriptor space)

- see Figure~\ref{fig:charness}

\paul{old:}

\mypara{Pose description}

- based mainly on robust joint-line distances (see appendix or add. material for details), results from Zhang et al.~\cite{geomfeatures:2017:wacv} suggest that these perform best among well-known pose descriptors.

- specialized for interactions with objects

\mypara{Scenelets}

- extracted by chopping up the full sequence of the recording into chunks of fixed location arc length at regular intervals

- each of these sub-sequences is sampled with regular spacing in descriptor-location space

- object histograms capture neighboring objects in a fixed-length feature (max over all objects: max of: fraction of bin covered by object, fraction of object covered by bin)

\mypara{Characteristic scenelets}

- some pose sequences do not give evidence of neighboring objects (e.g. walking next to an object), we want to filter out these pose sequences.

- some neighboring objects are not characteristic for a pose sequence (even if the pose sequence is characteristic for other neighboring objects), we want to filter out these objects

- so we want to find pairs of pose sequences and neighboring objects that occur often in the dataset

- object characteristicness: density of object histogram bins in descriptor space given the pose (factor out density of poses), = weighted average of object histogram bins in descriptor space


==> junk_oldText.tex <==
\section{Evaluation} \label{sec:evaluation}





\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{interactionAssisted/images/qualitativeA.pdf}
    \vspace{2in}
    \caption{Qualitative comparisons to state-of-the-art object detection methods. Our approach allows us to synthesize scenes that plausibly match the video, even in sequences where objects and the human performance are occluded.}
    \label{fig:qualitativeObject}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{interactionAssisted/images/qualitativeB.pdf}
    \vspace{6in}
    \caption{Qualitative comparisons to state-of-the-art pose detection methods.}
    \label{fig:qualitativePose}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{interactionAssisted/images/scene_evolution.pdf}
    \caption{Scenes can be explored over time. We show results of four different videos taken from the same scene. As interactions with more objects are made available, we can recompute the results to synthesize additional objects. Variations of scene explorations, for example performing the interactions in reverse order, as shown in the bottom row, give slightly different, but comparable and plausible results.
    }
    \label{fig:scene_evolution}
\end{figure}

\begin{figure}
%   \includegraphics[width=\columnwidth]{images/charness.pdf}
  \vspace{2in}
  \caption{VNect comparison.}
  \label{fig:vnect comparison}
\end{figure}

\mypara{Does joint estimation improve pose estimation and/or scene prediction?}
a) pose estimation: 2D vs 3D; Fig
b) compare against depth estimation also RCNN Fig; sigg17 comparison (vnect) 
\vspace{1in}


\mypara{Does perturbations of path traced  adversely affect output?}
a) synthetic perturbations in 2D FP; Fig
b) time variations; Fig
\vspace{1in}


\mypara{Ablation study}
effects of various terms; Fig
\vspace{1in}

\begin{figure}
%   \includegraphics[width=\columnwidth]{images/charness.pdf}
  \vspace{2in}
  \caption{Ablation study.}
  \label{fig:ablation}
\end{figure}




\mypara{Effect of increasing interaction over time.}
Figure; timelapse
\vspace{1in}


\mypara{qualitative versus quantitative evaluation.}
a. 2D input (not video) -> 3D pose + object locations .. evaluate consistency + plausibility;
b. test on synthetic data?





Scenes to be used for evaluation ($+$ means results are available $++$ means all visualizations have been computed $+++$ means they are in the paper - not all of them need to be in the paper):
\begin{itemize}
    \item $+$ lobby11
    \item $+$ lobby12
    \item $+$ lobby15
    \item $+$ lobby18-1
    \item $+++$ lobby19-3
    \item $+$ lobby22-1
    \item office1-1
    \item office2-1
    \item $+$ livingroom00
    \item $+$ garden1
\end{itemize}

Figures planned:
\begin{itemize}
    \item showing input path evolution: local, global, final/optimized
    \item pipeline figure
    \item video: input, input 2D, denis 3D projected to 2D; ours projected to 2D; ours projected to 2D + objects; ours from another view; static image with trace of path 
    \item table with scene complexity (number of frames, number of objects, average confidence)
\end{itemize}

Evaluation planned (+ means evaluation is set up and ready to go, ++ means evaluation is done for our results, +++ means evaluation is in the paper)
\begin{itemize}
    \item different interaction: shelf or white board
    \item $+$ improvement over object detectors: FRCNN, Monocular depth
    \item $+$ improvement over pose detectors: Denis et al. 2D and 3D pose
    \item 2 people
    \item \sout{over time .. evolving results with multiple sits, etc.} (more or less included in the path variation figure)
    \item if extra time, show result on synthetic input (2D fps)
\end{itemize}

\begin{table}[]
    \centering
    \caption{A frame is occluded, if any of the 14 2D features are occluded in the RGB image (human inspection GT).}
    \footnotesize
    \begin{tabular}{l|r|r|r|r|r}
        scene & length & occluded & frac. & objects & \\
        \hline
        \hline
        lobby11-couch       &  80 &   0 &   0.00 & 1 & Fig. \ref{fig:qualitativeObject} row 1 \\
        lobby24-3-3         &  49 &  41 &  0.84 & 4 & Fig. \ref{fig:scene_evolution} top left\\
        lobby12- & 130 &  74 &  0.57 & 2 & Fig. \ref{fig:qualitativeObject} row 2 \\
        lobby19-3           & 115 &  89 &  0.77 & 2 & Fig. \ref{fig:qualitativeObject} row 4 \\
        lobby18-1           & 120 &  98 &  0.82 & 1 & Fig. \ref{fig:qualitativeObject} row 3 \\
        lobby24-3-1         & 148 & 137 &  0.93 & 4 & Fig. \ref{fig:scene_evolution} topR \\
        lobby15             & 254 & 164 &  0.65 & 3 & ?? \\
        lobby24-3-2         & 182 & 182 & 1.00 & 4 & Fig. \ref{fig:scene_evolution} botL \\
        lobby24-2-2         & 189 & 185 &  0.98 & 4 & Fig. \ref{fig:scene_evolution} botR \\
        lobby22-1           & 224 & 218 &  0.97 & 4 & ?? \\
        library3            & 539 & 262 &  0.49 & 5 & ?? \\
        livingroom00        & 380 & 319 &  0.84 & 6 & Fig. \ref{fig:top_view} \\
        office1-1           & 348 & 347 & 1.00 & 7 & Fig. \ref{fig:teaser} \\
        garden1             & 430 & 369 &  0.86 & 5 & ?? \\ 
    \end{tabular}
    \label{tab:occlusions}
\end{table}


%%
%% Quantitative
%%


qualitative vs quantitative 

comment about im2cad or marr revisited


ablation




\mypara{Limitations.}
%
We currently assume the input camera to be fixed during the entire duration of the capture. Such a fixed viewpoint results in heavy occlusion in crowded scenes and makes the job of \name\ unnecessarily challenging. In large-scale environments, one can imagine having a network of fixed cameras to address this issue and jointly process the information from the individual cameras. 
%
An obvious limitation of \name\ is failing to react when it `sees' an interaction not in its interaction database. This is an unavoidable problem in any data-driven approach unless we  are able to additionally synthesize new interactions, which is a significantly more challenging problem. 
%
Furthermore, since we only rely on detected 2D joint locations from the monocular video, our method will fail when the 2D location detections are erroneous or if too much data is missing.
% partial signals can be confused with occlusions
%have only partial signals. 
%
Finally, since our method builds on the expectation that people react similarly in similar settings, it will naturally get confused when this assumption is broken. For example, a person decides to hand-walk, or uses the couch as a bed, \etc. We expect this to be partially addressed by richer interaction databases with associated probability priors on actions, and spatio-temporal  reasoning that detects and ignores `outlier' interactions by observing a scene over longer time intervals. 
